Preserving MWPM-Decodability in Fault-Equivalent Rewrites

Decoding a quantum error correction code is generally NP-hard, but corrections must be applied at a high frequency to suppress noise successfully. Matchable codes, like the surface code, exhibit a special structure that makes it possible to efficiently, approximately solve the decoding problem through minimum-weight perfect matching (MWPM). However, this efficiency-enabling property can be lost when constructing implementations for fault-tolerant gadgets such as syndrome-extraction circuits or logical operations. In this work, we take a circuit-centric perspective to formalise how the decoding problem changes when applying ZX rewrites to a ZX diagram with a given detector basis. We demonstrate a set of rewrites that preserve MWPM-decodability of circuits and show that these matchability-preserving rewrites can be used to fault-tolerantly extract quantum circuits from phase-free ZX diagrams. In particular, this allows us to build efficiently decodable, fault-tolerant syndrome-extraction circuits for matchable codes.

==> figures/matchability-preservation/generality/detector-partitioning.tex <==
\section{Detector partitioning}
\label{sec:mp:partition}
In the previous section, we have seen that we can decorate the $r_4$, $r_5$, and
$r_6$ rewrites to be matchability-preserving if the detector coverage of the
single spider is a subset of the flower or blossom shape.
The remaining cases will be covered in this section and we will show that we can
reduce each of these cases to spiders covered in blossom shapes under
conservative assumptions regarding the distance of the full diagram.
We call this process \emph{detector partitioning} and generalise it to deal with
any many-legged spider that is not covered in a subset of the flower or blossom
shape.

Consider the following matchable detector coverage of a four-legged spider,
which is made up of two ``double detectors'', that is, Pauli webs that are
contained twice in the Pauli web multiset. 
\begin{equation}
    \label{eq:mp:r4-dd-diagram}
    \tikzfig{matchability-preservation/detector-partitioning/r4-dd-LHS}
\end{equation}

This Pauli web multiset neither has the flower nor the blossom shape discussed
in the previous section and indeed, any detector-aware rewrite based on $r_4$
will not preserve matchability.
This is because we need to ``route'' four non-detector Pauli webs between the
bottom and the top spiders, but we only have two vertical wires and the local
detector basis of the RHS covers both vertical wires once already. 
\begin{equation}
        \tikzfig{matchability-preservation/detector-partitioning/r4-dd-LHS}
        \stackrel{(r_4)}\circeq
        \tikzfig{matchability-preservation/detector-partitioning/r4-dd-RHS}
\end{equation} 

However, we can also use these double detectors to our advantage:
A fault made up of two $X$ edge flips on the wires covered by such a pair of
detectors is undetectable because detectors are only violated by odd numbers of
anticommuting edge flips.
If this weight-two fault is nontrivial in the full diagram, this would imply
$\distance(D) \leq 2$ for the entire circuit $D$ where the four-legged
spider occurred.
\begin{equation}
    \label{eq:mp:partitioning-distance}
    \tikzfig{matchability-preservation/detector-partitioning/r4-dd-LHS-XX-with-context}
    \neq
    \tikzfig{matchability-preservation/detector-partitioning/r4-dd-LHS-with-context}
    \quad
    \implies
    \distance\left(
        {\ }
        \tikzfig{matchability-preservation/detector-partitioning/r4-dd-LHS-with-context}
        {\ }
    \right)
    \leq 2
\end{equation}
But such a low distance is a rare (and unhelpful) property since many QEC codes
use the distance to argue about correctability; and this specific distance does
not imply the correctability of any error.
It is therefore reasonable to assume $\distance(D) > 2$.
By contraposition of \cref{eq:mp:partitioning-distance}, the $X \otimes X$ fault
must therefore be trivial in the context of the full diagram.
In the language of stabilisers, this means that $X \otimes X$ at the indicated
positions must be stabilised by $D$.

For contexts with this property, we can construct a new fault-equivalent
rewrite:
\begin{lemma}[Double-detector rewrite $r_{dd}$]
    \label{thm:rdd-fault-equivalent}
    For a ZX diagram $D$ that stabilises $X \otimes X$ on the internal wires,
    the following rewrite is fault-equivalent.
    \begin{equation}
        \tikzfig{matchability-preservation/detector-partitioning/r4-double-detector-rewrite-LHS}
        \quad\stackrel{(r_{dd})}{\hat=}\quad
        \tikzfig{matchability-preservation/detector-partitioning/r4-double-detector-rewrite-RHS}
    \end{equation}
    We will refer to this rewrite as the \emph{double-detector rewrite
    $r_{dd}$}.
\end{lemma}
\begin{proof}
    The ZX diagrams of this rewrite are equivalent through the spider fusion
    rule.
    For fault equivalence, we need to show that all undetectable faults on the
    left-hand side have an equivalent fault with less or equal weight on the
    right-hand side, and vice versa.
    For the first direction, we realise that all wires on the left-hand side of
    the rewrite also exist on the right-hand side.
    Therefore, all faults have an identical equivalent in this direction.
    
    For the other direction, we consider an arbitrary fault $F$.
    If this fault contains a $Z$ flip on the new wire, we can push out the $Z$
    flip to observe that it's equivalent to an error on an external wire which
    also exists in the LHS diagram.
    \begin{equation}
        \tikzfig{matchability-preservation/detector-partitioning/r4-double-detector-rewrite-RHS-Z}
        \quad=\quad
        \tikzfig{matchability-preservation/detector-partitioning/r4-double-detector-rewrite-RHS-Z-pushout}
    \end{equation}
    If $F$ contains an $X$ fault, we can push it through the left spider to
    get the $X \otimes X$ fault that is stabilised by the context $D$.
    \begin{equation}
        \tikzfig{matchability-preservation/detector-partitioning/r4-double-detector-rewrite-RHS-X}
        \quad=\quad
        \tikzfig{matchability-preservation/detector-partitioning/r4-double-detector-rewrite-RHS-X-pushout}
        \quad=\quad
        \tikzfig{matchability-preservation/detector-partitioning/r4-double-detector-rewrite-RHS}
    \end{equation}
    As $D$ absorbs this error, $X$ flip too was trivial.
    If $F$ contains a $Y$ fault on the new wire, this is equivalent to an $X$
    and a $Z$ fault occuring on the internal wire but we have previously argued
    that the $X$ flip is trivial, so the $Y$ flip is equivalent to the $Z$ flip
    which we discussed before.
    All other wires also exist in the LHS diagram and we can therefore apply the
    identical fault on the LHS.
\end{proof}

This rewrite looks different from the ZX rewrites that we are used to because it
leaves the context $D$ unspecified, except for the stabiliser condition.
This raises the question of how such a rewrite should be applied.
We consider the part of the rewrite that isn't the context $D$ the interesting
part of the rewrite -- this is where the change to the diagram happens.
When considering whether we can apply this rewrite, we try to find the changing
part somewhere in a diagram and then search the remaining diagram for a suitable
context.
We then pick the context $D$ to be large enough that it includes the required
stabilising Pauli web\footnote{
    The performance of automated rewriting may benefit from choosing a minimal
    context to avoid wasting resources.
    For the theory, we can also just pick the entire diagram, as long as it has
    the desired property.
}.
Crucially, finding such a suitable context can be done in polynomial time over
the diagram size, so it is efficient enough to be used during compilation
\cite{bombin_unifying_2024,borghans_zx-calculus_2019}.

\begin{proposition}[Double-detector rewrite preserves matchability]
    \label{thm:mp:dd-rewrite-matchability}
    Let $D, D_1$ be ZX diagrams with a matchable detector basis $S_1$ of
    $D(D_1)$ such that $\distance(D(D_1)) > 2$,
    \begin{equation}
        D_1 = \tikzfig{matchability-preservation/detector-partitioning/four-legged}
        \quad
        \text{ and }
        \quad
        \tikzfig{matchability-preservation/detector-partitioning/four-legged-dd} \subseteq S_1[D_1]\,.
    \end{equation}

    Then there exists a Pauli web multiset $S_2$ for $D(D_2)$ and
    \begin{equation}
        D_2 = \tikzfig{matchability-preservation/detector-partitioning/rdd-inner-RHS}
    \end{equation}
    such that $S_1[D] = S_2[D]$ and $(D(D_1), S_1) \circeq (D(D_2), S_2)$
    preserves matchability.
\end{proposition}
\begin{proof}
    As we assumed $S_1$ to be matchable and the indicated wires of $D_1$ are
    already covered by two detectors, there cannot be any other detectors
    covering these wires.
    Therefore, an $X \otimes X$ fault on these wires is undetectable.
    As $\distance(D(D_1)) > 2$, this fault must be equivalent to the trivial
    fault in $D(D_1)$.
    Then \cref{thm:rdd-fault-equivalent} implies that $D(D_1) \hat= D(D_2)$ is a
    fault-equivalent rewrite.

    As $D_2$ does not allow any local detectors, we can use
    \cref{thm:uniquely-detector-aware} to construct a unique Pauli web multiset
    $S_2'$ for $D_2$ such that $(D_1, S_1[D_1]) \circeq (D_2, S_2')$ is a
    detector-aware rewrite.
    We can apply this detector-aware rewrite to $(D(D_1), S_1)$ following
    \cref{thm:det-aware-rewrites-compose} to get a Pauli web multiset $S_2$ for
    $D(D_2)$ such that $S_2[D] = S_1[D]$, $S_2[D_2] = S_2'$ and
    $(D(D_1), S_1) \circeq (D(D_2), S_2)$ is a detector-aware rewrite.

    We already know that $D(D_1) \hat= D(D_2)$ is fault-equivalent and $S_1$ is
    matchable, so the last thing we need to prove is $S_2$'s matchability.
    $S_2[D] = S_1[D]$ is matchable by assumption.
    $D$ includes the boundary wires of $D_2$, so we just need to check the
    internal wire of $D_2$.
    But as we can push out $X$ flips on the internal wire to become
    $X \otimes X$ faults, which are known to be trivial, the $X$ flip is trivial
    too and cannot violate any detectors.
    Therefore $S_2$ is matchable and we conclude that
    $(D(D_1), S_1) \circeq (D(D_2), S_2)$ is a matchability-preserving rewrite.
\end{proof}

This result allows us to decompose four-legged spiders for Pauli web multisets
that are not in the flower or blossom shape from \cref{sec:mp:ring-rewrites}.
For the example diagram in \cref{eq:mp:r4-dd-diagram} that we could not rewrite
matchability-preservingly with the $r_4$ rewrite, we can now apply this
alternative rewrite, assuming it occured in some diagram with a higher distance
than two.
\begin{equation}
    \tikzfig{matchability-preservation/detector-partitioning/r4-dd-LHS-with-context}
    \eqcirc
    \tikzfig{matchability-preservation/detector-partitioning/r4-dd-RHS-with-context}
\end{equation}

We can generalise this partitioning result to larger groups of Pauli webs as
follows:
\begin{proposition}[Generalised double-detector rewrite]
    \label{thm:generalised-partitioning}
    Let $D, D_1$ be ZX diagrams with a matchable detector basis $S_1$ of
    $D(D_1)$ such that $\distance(D(D_1)) > n$,
    \begin{equation}
        D_1 = \tikzfig{matchability-preservation/detector-partitioning/generalised-partitioning-D1}\,.
    \end{equation}
    Furthermore, let $E_l \subseteq E(D_1)$ be $n$ left edges of $D_1$ and let
    the following condition hold:
    \begin{equation}
        \label{eq:mp:generalised-partitioning-conditions}
        \left\{ \left\{ P \in S_1[D_1] \mid \exists e \in E_l : P(e) = Z \right\} \right\} \subseteq \tikzfig{matchability-preservation/detector-partitioning/generalised-partitioning-group}\,.
    \end{equation}
    Then there exists a Pauli web multiset $S_2$ for $D(D_2)$ and
    \begin{equation}
        D_2 = \tikzfig{matchability-preservation/detector-partitioning/generalised-partitioning-D2}
    \end{equation}
    such that $S_1[D] = S_2[D]$ and $(D(D_1), S_1) \circeq (D(D_2), S_2)$
    preserves matchability. 
\end{proposition}
\begin{proof}
    Let $D, D_1, S_1$ be as assumed in the claim.

    We first prove that $D(D_1)$ and $D(D_2)$ are fault-equivalent in analogy to 
    \cref{thm:rdd-fault-equivalent} and \cref{thm:mp:dd-rewrite-matchability}.
    For that, we notice that \cref{eq:mp:generalised-partitioning-conditions}
    ensures that each Pauli web covering the left boundary wires of $D_1$ in
    green covers exactly two of these edges in green.
    Therefore, the following weight-$n$ fault is undetectable in $D(D_1)$:
    \begin{equation}
        \tikzfig{matchability-preservation/detector-partitioning/generalised-partitioning-undetectable}
    \end{equation}
    Since $\distance(D(D_1)) > n$, this fault must be trivial.
    We can use this to prove fault equivalence between $D(D_1)$ and $D(D_2)$ by
    pushing out all undetectable, internal edge flips of $D_1$ to edges of $D$
    without increasing their weight:
    \begin{equation}
        \begin{gathered}
            \tikzfig{matchability-preservation/detector-partitioning/generalised-partitioning-X-pushout-1}
            =
            \tikzfig{matchability-preservation/detector-partitioning/generalised-partitioning-X-pushout-2}
            =
            \tikzfig{matchability-preservation/detector-partitioning/generalised-partitioning-X-pushout-3}
            \\[8pt]
            \tikzfig{matchability-preservation/detector-partitioning/generalised-partitioning-Z-pushout-1}
            =
            \tikzfig{matchability-preservation/detector-partitioning/generalised-partitioning-Z-pushout-2}
        \end{gathered}
    \end{equation}

    Second, we lift this fault-equivalent rewrite to be a
    matchability-preserving rewrite in analogy to
    \cref{thm:mp:dd-rewrite-matchability}.
    To do so, we realise that $D_2$ permits no local detectors, so there must
    exist a unique Pauli web multiset $T$ for $D_2$ such that
    $(D_1, S_1[D_1]) \circeq (D_2, T)$ is a detector-aware rewrite
    (\cref{thm:uniquely-detector-aware}).
    We apply this detector-aware rewrite to $(D(D_1), S_1)$ using
    \cref{thm:det-aware-rewrites-on-det-basis} to obtain a detector basis $S_2$
    for $D(D_2)$ such that $(D(D_1), S_1) \circeq (D(D_2), S_2)$ is a
    detector-aware rewrite and $S_1[D] = S_2[D]$, $S_2[D_2] = T$ hold.
    $S_2[D]$ is matchable because $S_1[D]$ was matchable.
    The only wire in $D(D_2)$ that was not already in $D$ is the internal wire
    of $D_2$.
    Any green Pauli web covering this internal wire must also cover a left and a
    right boundary wire of $D_2$ nontrivially.
    But \cref{eq:mp:generalised-partitioning-conditions} ensures that $S_2$
    contains no such Pauli web.
    
    We conclude that $(D(D_1), S_1) \circeq (D(D_2), S_2)$ is a
    matchability-preserving rewrite.
\end{proof}

Using this generalisation, we can now rewrite four-to-six-legged spiders under
arbitrary matchable Pauli web coverage, assuming a global distance of two or
three.
This is because we found matchability-preserving decompositions for flower- and
blossom-shaped Pauli web coverages in \cref{sec:mp:ring-rewrites}.
Any Pauli web multiset that is in neither of these shapes can be partitioned
and we can use \cref{thm:generalised-partitioning} to ``pull out'' partitions
under the respective distance requirement.
The partitioning rewrite ensures that the partition that was pulled out now
covers another spider with less legs in the flower shape that was introduced
in the previous section.
The other spider in the decomposition may still not be in the blossom or flower
shape but it has one partition less than the original spider.
Repeated applications of the partitioning rule allow us ensure that all spiders
are covered in subsets of the blossom or flower shapes. 

For example, we can use a partitioning and the $r_4$ rewrite to
matchability-preservingly decompose the following five-legged spider with a
partitioned Pauli web multiset into spiders with at most three legs.
Here, the application of the partitioning rewrite requires the diagram to have
a distance of at least two.
\begin{equation}
    \tikzfig{matchability-preservation/detector-partitioning/r5-partitions-1}
    \stackrel{(r_{dd}^*)}\circeq
    \tikzfig{matchability-preservation/detector-partitioning/r5-partitions-2}
    \stackrel{(r_5)}\circeq
    \tikzfig{matchability-preservation/detector-partitioning/r5-partitions-3}
\end{equation}

